Pre-registration for Predictive Modeling

Amid rising concerns of reproducibility and generalizability in predictive modeling, we explore the possibility and potential benefits of introducing pre-registration to the field. Despite notable advancements in predictive modeling, spanning core machine learning tasks to various scientific applications, challenges such as overlooked contextual factors, data-dependent decision-making, and unintentional re-use of test data have raised questions about the integrity of results. To address these issues, we propose adapting pre-registration practices from explanatory modeling to predictive modeling. We discuss current best practices in predictive modeling and their limitations, introduce a lightweight pre-registration template, and present a qualitative study with machine learning researchers to gain insight into the effectiveness of pre-registration in preventing biased estimates and promoting more reliable research outcomes. We conclude by exploring the scope of problems that pre-registration can address in predictive modeling and acknowledging its limitations within this context.

==> 05_case_study.tex <==
\section{Case Study}
\jessica{
\begin{itemize}
    \item Several years ago we developed a statistical model to predict employee attitudes from communication data
    \item We followed the standard ML protocol, train/validate/test
    \item The initial models looked great, with 90\% precision and 60\% recall. Our internal HR team saw results and wanted to use the model
    \item Before handing it over, we decided to pre-register the model and test it on next year’s data, following our new proposed flow (Figure 1, Table 1)
    \item This had a few effects:
    \begin{itemize}
        \item Forced us to think hard about several aspects of our research design and evaluation
        \item Introduced challenges in how to pre-register complex model that uses private data
        \item Fundamentally changed the nature of our results
    \end{itemize}
    \item Pre-registered on OSF and tested
    \item Performance tanked, to 20\% precision (bit better than random guessing)
    \item Determined this was due to non-stationarity in how people are using email
\end{itemize}
}
